Rule-Guided Reinforcement Learning Policy Evaluation and Improvement

We consider the challenging problem of using domain knowledge to improve deep reinforcement learning policies. To this end, we propose LEGIBLE, a novel approach, following a multi-step process, which starts by mining rules from a deep RL policy, constituting a partially symbolic representation. These rules describe which decisions the RL policy makes and which it avoids making. In the second step, we generalize the mined rules using domain knowledge expressed as metamorphic relations. We adapt these relations from software testing to RL to specify expected changes of actions in response to changes in observations. The third step is evaluating generalized rules to determine which generalizations improve performance when enforced. These improvements show weaknesses in the policy, where it has not learned the general rules and thus can be improved by rule guidance. LEGIBLE supported by metamorphic relations provides a principled way of expressing and enforcing domain knowledge about RL environments. We show the efficacy of our approach by demonstrating that it effectively finds weaknesses, accompanied by explanations of these weaknesses, in eleven RL environments and by showcasing that guiding policy execution with rules improves performance w.r.t. gained reward.

==> figures/important.tex <==
\begin{tikzpicture}[scale = 0.15]

% Draw the triangular shape with rounded corners
\draw[very thick, red, fill=white, line join=round] (0,0) -- (3,5.196) -- (6,0) -- cycle;

% Add a text label inside the triangle (optional)
\node at (3.5,1.5) {\Large\textbf{!}};

\end{tikzpicture}

==> figures/monitor.tex <==
\begin{tikzpicture}[scale = 0.22]

% Draw the box
\draw[thick] (0,0) rectangle (5,5);

% Coordinates for the magnifying glass
\coordinate (center) at (2.5,2.5);
\coordinate (handle_start) at (0.5,0.5);
\coordinate (handle_end) at (1.9,1.9);

% Draw the magnifying glass lens
\shade[ball color=white,opacity=0.5] (center) circle (1.2); % Glass with shading
\draw[thick] (center) circle (1.2); % Outer circle

% Draw the handle
\draw[very thick, fill=gray] (handle_start) -- ++(0.2,0.2) -- (handle_end) -- ++(-0.2,-0.2) -- cycle; % Handle

% Add some shine to the glass
\begin{scope}
    \clip (center) circle (1.2);
    \draw[white,opacity=0.5] (2,3.5) arc[start angle=150,end angle=250,radius=1.5];
\end{scope}

% Add a small circle inside to create the effect of a rim
\draw[thick, color=black] (center) circle (1);

\begin{pgfonlayer}{background}
\node[]at(0.3,2.5){
\begin{tikzpicture}[scale=0.15]
\draw[step=1cm,black,very thin] (0,0) grid (5,5);
\fill[blue] (0,1) rectangle (1,2);
\fill[red] (2,3) rectangle (3,4);
\fill[green](3,0) rectangle (4,1);
\end{tikzpicture}
};
\end{pgfonlayer}

\end{tikzpicture}

==> tables/rule_guided.tex <==

\begin{table*}[t]  
    \begin{tabular}{l|l|l|l|l|l|l|l}
    \multirow{2}{*}{Experiment} & \multirow{2}{*}{Base} & \multicolumn{3}{|c|}{Rule-Guided} & \multicolumn{3}{|c}{Extended} \\ \cline{3-8}
    & & min. & mean & max. & min. & mean & max. \\ \hline  small & 1073.02& 1223.11& 1250.35& 1280.80& 1023.31& 1048.96& 1101.04 \\ \hline 
 small(NC) & 455.43& 574.27& 581.27& 589.39& 378.84& 401.42& 420.07 \\ \hline 
 medium & 1317.59& 1508.73& 1543.94& 1562.62& 1308.80& 1368.72& 1443.91 \\ \hline 
 medium(NC) & 854.20& 1064.88& 1084.63& 1101.49& 797.98& 827.87& 865.53 \\ \hline 
 original & 1562.80& 1701.15& 1809.30& 1899.43& 1480.66& 1518.03& 1556.39 \\ \hline 
 original(NC) & 833.65& 1062.53& 1112.57& 1163.20& 737.59& 781.10& 825.16 \\  

    \end{tabular}
    \caption{Cumulative reward from evaluation of RL policies in six PAC-Man levels. Base denotes basic training for $5 \cdot 10^6$ steps (original and original (NC)), or $2.5 \cdot 10^6$ steps (other levels), rule-guided extended, standard extended training, each for $10^6$ steps.}
    \label{tab:rule-guided_pacman_performance}
\end{table*}


==> tables/weaknesses_hw.tex <==
\begin{table}[t]
\footnotesize
\centering
 
 %         \begin{tabular}{l|c|c|c|c|c|c}
 %         \multirow{2}{*}{Experiment} &  \multicolumn{3}{|c|}{Detected Weaknesses} & \multicolumn{3}{|c}{\# Evaluations} \\ \cline{2-7}
 %          & min. & mean & max. & min. & mean & max. \\ \hline 
 %           highway & \makecell{$0.04$ \\ $0.00$ }& \makecell{ $0.51$ \\ $0.09$ }& \makecell{ $0.77$ \\ $0.26$ } & $74.0$ & $90.8$ & $112.0$\\ \hline 
 % highway-fast & \makecell{$0.23$ \\ $0.00$ }& \makecell{ $0.60$ \\ $0.12$ }& \makecell{ $0.85$ \\ $0.36$ } & $92.0$ & $110.0$ & $132.0$\\ \hline 
 % merge & \makecell{$0.40$ \\ $0.08$ }& \makecell{ $0.62$ \\ $0.20$ }& \makecell{ $0.90$ \\ $0.46$ } & $42.0$ & $109.6$ & $158.0$\\ \hline 
 % intersection & \makecell{$0.21$ \\ $0.00$ }& \makecell{ $0.52$ \\ $0.15$ }& \makecell{ $0.91$ \\ $0.50$ } & $12.0$ & $20.8$ & $26.0$\\ \hline 
 % roundabout & \makecell{$0.44$ \\ $0.06$ }& \makecell{ $0.62$ \\ $0.18$ }& \makecell{ $0.73$ \\ $0.38$ } & $16.0$ & $33.6$ & $54.0$\\  
 %         \end{tabular}

         \begin{tabular}{l|c|c|c|c|c|c}
         \multirow{2}{*}{Experiment} &  \multicolumn{3}{|c|}{Detected Weaknesses} & \multicolumn{3}{|c}{\# Evaluated Rules} \\ \cline{2-7}
          & min. & mean & max. & min. & mean & max. \\ \hline 
           highway & $0.00$ & $0.05$ & $0.16$  & $74.0$ & $90.8$ & $112.0$\\ \hline 
 highway-fast & $0.00$ & $0.08$ & $0.25$  & $92.0$ & $110.0$ & $132.0$\\ \hline 
 merge & $0.07$ & $0.16$ & $0.37$  & $42.0$ & $109.6$ & $158.0$\\ \hline 
 intersection & $0.00$ & $0.11$ & $0.40$  & $12.0$ & $20.8$ & $26.0$\\ \hline 
 roundabout & $0.03$ & $0.14$ & $0.38$  & $16.0$ & $33.6$ & $54.0$\\  

         \end{tabular}
         
              \caption{Detected weaknesses and number of evaluations in five \texttt{highway-env} environments.}
    \label{tab:weaknesses-hw}
\end{table}


==> tables/weaknesses_pac.tex <==
\begin{table}[t]
\centering
\footnotesize
    

 %         \begin{tabular}{l|c|c|c|c|c|c}
 %         \multirow{2}{*}{Experiment} &  \multicolumn{3}{|c|}{Detected Weaknesses} & \multicolumn{3}{|c}{\# Evaluations} \\ \cline{2-7}
 %          & min. & mean & max. & min. & mean & max. \\ \hline 
 %           small & \makecell{$0.20$ \\ $0.02$ }& \makecell{ $0.56$ \\ $0.16$ }& \makecell{ $0.82$ \\ $0.38$ } & $85.0$ & $105.4$ & $119.0$\\ \hline 
 % small-nc & \makecell{$0.18$ \\ $0.05$ }& \makecell{ $0.35$ \\ $0.13$ }& \makecell{ $0.66$ \\ $0.36$ } & $73.0$ & $85.0$ & $97.0$\\ \hline 
 % medium & \makecell{$0.40$ \\ $0.04$ }& \makecell{ $0.49$ \\ $0.11$ }& \makecell{ $0.64$ \\ $0.21$ } & $106.0$ & $117.6$ & $133.0$\\ \hline 
 % medium-nc & \makecell{$0.17$ \\ $0.01$ }& \makecell{ $0.30$ \\ $0.11$ }& \makecell{ $0.54$ \\ $0.29$ } & $93.0$ & $109.6$ & $126.0$\\ \hline 
 % original & \makecell{$0.38$ \\ $0.04$ }& \makecell{ $0.56$ \\ $0.18$ }& \makecell{ $0.88$ \\ $0.49$ } & $98.0$ & $121.6$ & $144.0$\\ \hline 
 % original-nc & \makecell{$0.17$ \\ $0.06$ }& \makecell{ $0.43$ \\ $0.16$ }& \makecell{ $0.60$ \\ $0.24$ } & $102.0$ & $108.8$ & $113.0$\\  

 %         \end{tabular}

         \begin{tabular}{l|c|c|c|c|c|c}
         \multirow{2}{*}{Experiment} &  \multicolumn{3}{|c|}{Detected Weaknesses} & \multicolumn{3}{|c}{\# Evaluated Rules} \\ \cline{2-7}
          & min. & mean & max. & min. & mean & max. \\ \hline 
           small & $0.01$ & $0.13$ & $0.31$  & $85.0$ & $105.4$ & $119.0$\\ \hline 
 small-nc & $0.05$ & $0.11$ & $0.30$  & $73.0$ & $85.0$ & $97.0$\\ \hline 
 medium & $0.03$ & $0.08$ & $0.15$  & $106.0$ & $117.6$ & $133.0$\\ \hline 
 medium-nc & $0.01$ & $0.09$ & $0.23$  & $93.0$ & $109.6$ & $126.0$\\ \hline 
 original & $0.04$ & $0.16$ & $0.44$  & $98.0$ & $121.6$ & $144.0$\\ \hline 
 original-nc & $0.06$ & $0.14$ & $0.22$  & $102.0$ & $108.8$ & $113.0$\\ 
         \end{tabular}
         

         \caption{Detected weaknesses and number of evaluations in six PAC-Man levels.}
    \label{tab:weaknesses-pac}
\end{table}


==> tikz_config.tex <==
\usetikzlibrary{fit,arrows.meta,external, positioning,shapes,shapes.arrows}
\usepackage{pgfplots}
\makeatletter
\tikzset{
    database top segment style/.style={draw},
    database middle segment style/.style={draw},
    database bottom segment style/.style={draw},
    database/.style={
        path picture={
            \path [database bottom segment style]
                (-\db@r,-0.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database middle segment style]
                (-\db@r,0.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database top segment style]
                (-\db@r,1.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database top segment style]
                (0, 1.5*\db@sh) circle [x radius=\db@r, y radius=\db@ar*\db@r];
        },
        minimum width=2*\db@r + \pgflinewidth,
        minimum height=3*\db@sh + 2*\db@ar*\db@r + \pgflinewidth,
    },
    database segment height/.store in=\db@sh,
    database radius/.store in=\db@r,
    database aspect ratio/.store in=\db@ar,
    database segment height=0.1cm,
    database radius=0.25cm,
    database aspect ratio=0.35,
    database top segment/.style={
        database top segment style/.append style={#1}},
    database middle segment/.style={
        database middle segment style/.append style={#1}},
    database bottom segment/.style={
        database bottom segment style/.append style={#1}}
}
\makeatother

\colorlet{myred}{red!80!black}
\colorlet{myblue}{blue!80!black}
\colorlet{mygreen}{green!60!black}
\colorlet{myorange}{orange!70!red!60!black}
\colorlet{mydarkred}{red!30!black}
\colorlet{mydarkblue}{blue!40!black}
\colorlet{mydarkgreen}{green!30!black}
\tikzstyle{node}=[thick,circle,draw=myblue,minimum size=22,inner sep=0.5,outer sep=0.6]
\tikzstyle{node in}=[node,green!20!black,draw=mygreen!30!black,fill=mygreen!25]
\tikzstyle{node hidden}=[node,blue!20!black,draw=myblue!30!black,fill=myblue!20]
\tikzstyle{node convol}=[node,orange!20!black,draw=myorange!30!black,fill=myorange!20]
\tikzstyle{node out}=[node,red!20!black,draw=myred!30!black,fill=myred!20]
\tikzstyle{connect}=[thick,mydarkblue] %,line cap=round
\tikzstyle{connect arrow}=[-{Latex[length=4,width=3.5]},thick,mydarkblue,shorten <=0.5,shorten >=1]
\tikzset{ % node styles, numbered for easy mapping with \nstyle
  node 1/.style={node in},
  node 2/.style={node hidden},
  node 3/.style={node out},
}
\def\nstyle{int(\lay<\Nnodlen?min(2,\lay):3)} 

\usepgfplotslibrary{groupplots}
    \pgfplotsset{
        % use this `compat` level or higher to get this result
        compat=newest,
        every axis label={font=\footnotesize}, % set the axis label font to 10pt
        tick label style={
            font=\footnotesize,     % set the tick label font to 8pt
        },
    }
\pgfplotsset{
    compat=newest,
    /pgfplots/legend image code/.code={%
        \draw[mark repeat=2,mark phase=2,#1] 
            plot coordinates {
                (0cm,0cm) 
                (0.15cm,0cm)
                (0.3cm,0cm)%
            };
    },
}
\pgfplotsset{every x tick label/.append style={font=\footnotesize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\footnotesize, xshift=0.5ex}}
\pgfplotsset{every xlabel label/.append style={font=\footnotesize}}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground} 

